Hallucination-Free GUI Grounding via Regression-Free Layout-Aware Matching

GUI agents are shifting from metadata-dependent large language models to purely visual multimodal large language models (MLLMs) that operate directly on screenshots. The core task, GUI grounding, requires translating abstract user instructions into precise element coordinates. This task faces a persistent dual obstacle: conventional grounding models lack the semantic richness to interpret abstract instructions, while end-to-end MLLMs suffer from coordinate hallucinations caused by deficient fine-grained perception. We propose a regression-free framework where a frozen MLLM performs instruction parsing and a dedicated grounding model handles precise localization without learning any coordinate regression. A frozen MLLM first elaborates the abstract instruction into a structured visual description rich in layout cues. These descriptions are then fed to a novel Layout-Aware GUI Grounding Model, which performs regression-free localization by matching against layout-prior candidates, inherently suppressing hallucinations and avoiding expensive fine-tuning. The grounding model is trained with only Text/Icon binary labels, requiring no coordinate regression parameters. On ScreenSpot-Pro, our method achieves over 20% improvement in grounding accuracy over end-to-end systems; on Mind2Web, it raises success rate and element selection rate by more than 15%. These results demonstrate that decoupling instruction understanding from layout-aware localization effectively resolves the core challenges of GUI interaction.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly state the three contributions (Layout-Aware GUI Grounding Model, layout-prior injection and geometric fusion mechanism, decoupled intent-driven grounding framework), and the experimental results on ScreenSpot-Pro and Mind2Web directly support the claimed accuracy improvements. The scope is explicitly limited to GUI visual grounding tasks.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper notes that the training-free MLLM may lack task-specific optimization compared to fine-tuned models, which is reflected in narrower Operation F1 score gains. The dependency on pre-trained CLIP features and DINO detection may also limit performance on highly non-standard or heavily customized interfaces.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not include theoretical results or formal proofs. The contributions are primarily methodological and empirical.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper?
    \item[] Answer: \answerYes{}
    \item[] Justification: Training details are provided in Section 3.4, including dataset construction (200k images from public GUI datasets, parsing tools, Qwen3-VL caption generation), model architecture (DINO detector with Swin-Tiny backbone, CLIP ViT-B/32), hyperparameters (learning rates, batch sizes, epochs, optimizer settings), and hardware configuration (8 RTX 3090 GPUs). The loss functions for both stages are formally defined with equations.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code?
    \item[] Answer: \answerNo{}
    \item[] Justification: Code and processed datasets are not publicly released at submission time to preserve anonymity. They will be made publicly available upon paper acceptance.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 3.4 provides complete training details including data splits (9:1), all hyperparameters with exact values, optimizer choices (AdamW for Stage 1, Adam for Stage 2), learning rate schedules (cosine annealing), and evaluation protocols. Three query subsets (simple, compound, spatial) are defined for fine-grained analysis.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Due to computational constraints (each full training run requires approximately 120 GPU-hours on 8 RTX 3090 GPUs), we report single-run results following common practice in the GUI grounding literature. We acknowledge this limitation and encourage future work to conduct multi-run statistical validation.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 3.4 specifies hardware (8 NVIDIA GeForce RTX 3090 GPUs), training duration (50 epochs for Stage 1, 20 epochs for Stage 2), batch sizes (effective batch size 8 for Stage 1, 256 for Stage 2), and total GPU-hours (approximately 120 GPU-hours per full training run).

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research uses publicly available benchmark datasets (ScreenSpot-Pro, Mind2Web) and open-source models (DINO, CLIP, Qwen-VL). No human subjects data was collected. We have reviewed the NeurIPS Code of Ethics and believe this work complies with all guidelines.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper discusses positive impacts including improved accessibility and productivity through more reliable GUI agents. Potential negative impacts include enabling automated manipulation of web interfaces for malicious purposes (e.g., automated fraud, scraping). We suggest limiting release to research purposes and encouraging responsible deployment guidelines.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse?
    \item[] Answer: \answerNA{}
    \item[] Justification: The proposed model is a specialized GUI grounding component, not a general-purpose generative model. Its localization outputs are task-specific and do not pose the same misuse risks as generative language or image models. No high-risk data or models are released.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All used datasets (ScreenSpot, Mind2Web) and pre-trained models (DINO, CLIP, BERT, Qwen-VL) are properly cited with their original papers. Datasets and models used are publicly available under their respective licenses (e.g., MIT, CC-BY, Apache 2.0).

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: At submission time, no new assets (datasets, pre-trained model checkpoints) are publicly released. Documentation will be provided upon release after acceptance.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve crowdsourcing or research with human subjects. All experiments use existing benchmark datasets.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve human subjects research. No IRB approval was required.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerYes{}
    \item[] Justification: The MLLM (Qwen-VL, GPT-4V) is a core component of the proposed framework, serving as the instruction elaboration module. Its role, configuration, and training-free nature are described in Sections 3.2 and 3.4. The MLLM is used in a frozen, inference-only manner.

\end{enumerate}
